Proteus: Enabling High-Performance Processing-Using-DRAM with Dynamic Bit-Precision, Adaptive Data Representation, and Flexible Arithmetic

Processing-using-DRAM (PUD) is a paradigm where the analog operational properties of DRAM are used to perform bulk logic operations. While PUD promises high throughput at low energy and area cost, we uncover three limitations of existing PUD approaches that lead to significant inefficiencies: (i) static data representation, i.e., two's complement with fixed bit-precision, leading to unnecessary computation over useless (i.e., inconsequential) data; (ii) support for only throughput-oriented execution, where the high latency of individual PUD operations can only be hidden in the presence of bulk data-level parallelism; and (iii) high latency for high-precision (e.g., 32-bit) operations. To address these issues, we propose Proteus, the first hardware framework that addresses the high execution latency of bulk bitwise PUD operations by implementing a data-aware runtime engine for PUD. Proteus reduces the latency of PUD operations in three different ways: (i) Proteus dynamically reduces the bit-precision (and thus the latency and energy consumption) of PUD operations by exploiting narrow values (i.e., values with many leading zeros or ones); (ii) Proteus concurrently executes independent in-DRAM primitives belonging to a single PUD operation across multiple DRAM arrays; (iii) Proteus chooses and uses the most appropriate data representation and arithmetic algorithm implementation for a given PUD instruction transparently to the programmer.

==> sections/04-implementation_old.tex <==
\vspace{-10pt}
\section{\prop Implementation}
\label{sec:implementation}


\subsection{Subarray Organization}
\label{sec:implementation:subarray}

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/subarray_org-crop.pdf}
    \caption{}
    \label{fig:implementation:subarray}
%    \vspace{-4mm}
\end{figure}


\subsection{Parallelism-Aware \uprog Library}
\label{sec:implementation:library}


\subsection{Dynamic Bit-Precision Engine}
\label{sec:implementation:dynamic-precision}


\subsection{\uprog Selector Unit}
\label{sec:implementation:control-unit}

% \textit{
% outlines of implementation part, divided into 3 sections: 
% \begin{itemize}
%     \item Overview of SSL architecture 
%         \begin{itemize}
%             \item data layout required by SSL 
%             \item logic for in-DRAM-computing 
%             \item logic for subarray-level parallelism 
%             \item logic for moving data among subarrays (shifting carry) 
%             \item logic for transferring data between banks (for NNs) 
%             \item logic for data transposition from horizontal to SSL layout 
%         \end{itemize}
%     \item Various arithmetic approaches 
%         \begin{itemize}
%             \item a summary of different approaches 
%             \item bit-serial on SSL
%             \item bit-parallel
%             \item RB 
%             \item SIMDRAM approach 
%         \end{itemize}
%     \item Automatic tool 
%         \begin{itemize}
%             \item automatically find near-optimal implementation (i.e. arithmetic operation, data allocation, etc.) of a workload - case study: gemv 
%             \item dynamic precision - case study: reduction 
%         \end{itemize}
%     % \item System integration 
% \end{itemize}
% } 



% \jgl{I think an overview section (with a good central figure) would be good. We are going to have many different things and we should help the reader to "navigate" over the paper.}

% % Likely divide into 2-3 sections.

% Do we need to show LISA shifts image, RB circuit image, SALP mechanism image ? \\
% Do we need to show AP and AAP operations performed by each algorithms ? \\

% We evaluated different algorithms based on the serial and parallelism available. Then we analyzed and find the best possible layouts for them to maximize their parallelism. 

% \subsection{Bitserial approaches}: 

% \jgl{Now it's time to give all these approaches proper names. SIMDRAM+SALP+LISA, for example, is not a good name. Let's start thinking what it is: it's a vertical layout that can operate in parallel on several bits.}

% \jgl{Btw, the substrate is different from the representation: 2's complement or RB.}

% \jgl{That is also different from the algorithm: bit serial, bit parallel. We will need a table or a figure to make all these different combinations clear.}

% \textbf{SIMDRAM addition} : In this we are directly using the current SOTA algorithm as presented in SIMDRAM. Assumption/Constraint here is that our DRAM substrate doesnt have any LISA transfer options and Subarray level parallelism(SALP). 

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/SIMDRAM.png}
%     \caption{SIMDRAM layout}
%     %A characteristic
%     %linear line is fitted
%     %along the area estimated for the transistor count.}
%     \label{fig:fitness}
% %    \vspace{-4mm}
% \end{figure}

% \textbf{SIMDRAM + SALP addition} : In this we are directly using the current SOTA algorithm as presented in SIMDRAM on multiple subarrays in DRAM in parallel usin SALP mechanism. Assumption/Constraint here is that our DRAM substrate doesnt have any LISA transfer options. 

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/SIMDRAM_SALP.png}
%     \caption{SIMDRAM + SALP layout}
%     %A characteristic
%     %linear line is fitted
%     %along the area estimated for the transistor count.}
%     \label{fig:fitness}
% %    \vspace{-4mm}
% \end{figure}


% \textbf{SIMDRAM + SALP + LISA addition}: In this we have the LISA transfer options available with subarray level parallelism. In this method we exploit the multiple subarrays and place the data according to the following figure and then can calculate the boolean/arithmetic operation based on the AP/AAPs cycles using the MAJ-NOT representation parallely across all used subarrays and then can transfer using LISA links. Adder used is the ripple carry adder which is represented in form of AND-OR gates and then MAJ-NOT gates and then minimized for minimum number of MAJ-NOT nodes and then represented in the optimal form of AP and AAP. 

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/SIMDRAM_SALP_LISA.png}
%     \caption{SIMDRAM + SALP + LISA layout}
%     %A characteristic
%     %linear line is fitted
%     %along the area estimated for the transistor count.}
%     \label{fig:fitness}
% %    \vspace{-4mm}
% \end{figure}

% \subsection{Bitparallel approaches}: 
% We come accross many approaches like Ladner Fischer adder, Kogge stone adder, Sklansky adder etc. and found out that Sklansky adder and Carry select adder turns out to be the best two candidate and others latency are less than the found one. 
% All bit parallel approaches uses SIMDRAM + SALP + LISA(SSL) mechanisms to effectively use the parallelism between the adders. 

% \textbf{Sklansky addition} :
% The layout of the following adder is specified in the following figure. Again the following gates will be converted to MAJ-NOT logic and optimized in such a way to give lowest AP/AAP's and can be transferred using LISA links.

% \textbf{Carry select addition}: 
% The layout of the following adder is specified in the following figure. In this approach, n bits are divided into chunks of 4bits and then SSL addition is performed and carry and sums to be muxed are transferred over LISA links to the appropriate the subarrays. 

% \textbf{RB adder}: 
% Redundant Binary representation doesn't require carry to be propagated and hence can use the parallelism effectively provided by the SALP mechanism. In this adder, no of boolean gates to be used are very high but after converting to MAJ-NOT representation and optimizing, it is effectively reduced to very less AP and AAP operations. Following is the layout for RB adder. IN RB representation, instead of 1, 0 we have four representation corresponding to 00 = 0 , 01 = 1 , 10 = -1, 11 = 0. and based on these we can write any binary number in RB format in terms of Xi+, Xi- and carry being generated as hi, fi. 


% First, microbenchmarking analysis of different precision, representation, operation, algorithm, etc. Analysis of transformation across data types and layouts (SIMDRAM, SIMDRAM+SALP, SIMDRAM+SALP+LISA...). 

% Second, pareto-optimal analysis, heuristics?

% Third, compiler analysis for adaptive data precision.

% Fourth, enhanced controller.

In this section, we discuss the architecture of \prop{} based on the previous works in section 4.1.1, and also explain the modified mechanism and new hardware introduced to support the implementation of real workloads in section 4.1.2 and 4.1.3. Then we discuss the implementation of different algorithms in section 4.2 and optimization in section 4.3 proposed from our software compiler to enhance the parallelism obtained our substrate. 
% First, we will look at what different components are proposed previously and are required by the \prop{}. 
% Then, we will discuss our emulator to evaluate the results.

% \subsection{Overview of \prop{}}

% \begin{figure*}[!htp]
%     \centering
%     \includegraphics[width=1.05\textwidth]{figures/overview.pdf}
%     \caption{\prop{} overview}
%     \label{fig:overview}
% %    \vspace{-4mm}
% \end{figure*}

% \jgl{The first five subsections are not an overview of \prop{}, but background on SALP, LISA, Ambit, and SIMDRAM.}
% \Mayank{Then, I think I should summarize them.}

% \subsubsection{Data Layout}: 
% We have done our analysis of the vertical data layout as proposed in the SIMDRAM framework \cite{hajinazarsimdram}, an end-to-end solution that enables users to implement arbitrary operations in DRAM using the AAP/AP \cite{seshadri2017ambit} command sequences. Our evaluation considers different algorithms implemented in SIMD fashion, with a transposition unit present in the memory controller for converting data into a vertical layout. 

% \subsubsection{Subarray level parallelism}: To operate multiple subarrays simultaneously, we will be utilizing the SALP (Subarray level parallelism) technique \cite{salp} proposed earlier. One of the SALP mechanisms we will be using is MASA (Multitudes of activated subarrays). The primary idea behind MASA is to enable the activation of multiple subarrays at the same time while allowing the memory controller to designate one specific subarray to drive the global bit lines during the next column command:

% It overlaps the activation of different subarrays within a bank. Just before issuing a column command to any of the activated subarrays, the memory controller designates one particular subarray whose row buffer should serve the column command. To implement this technique, the following changes need to be made to the DRAM microarchitecture, i) Addition of a designated-bit latch to each subarray, ii) Introduction of a new DRAM command, SA SEL (subarray-select), and iii) Routing of a new global wire (subarray-select).

% \jgl{Do we have an evaluation of total area overhead? Ideally, yes. And it would go at the end of the evaluation section.}

% \subsubsection{Copying and moving data among banks}: We will be utilizing the Rowclone method proposed earlier \cite{seshadri2013rowclone}, which involves two operations: FPM (Fast parallel mode) and PSM (Pipelined serial mode). FPM is used to copy data from the source row of one subarray to the destination row of the same subarray. This is done by pre-charging the source row and then activating the subarray to copy the data into the LRB (Local row buffer). Then, the destination row is activated, and the data is copied from the LRB to the destination row.

% PSM, on the other hand, is an extension of FPM, where the source row is precharged and activated to copy the data into the LRB. Then, the data is transferred from the LRB to the GRB (Global row buffer) before being copied to a different bank subarray LRB. Finally, the destination row is activated, and the data is copied from the source row of one subarray in one bank to the destination row of another subarray in a different bank.

% \subsubsection{Moving data among subarrays}: The LISA (Low-cost interlinked subarrays) \cite{chang2016low} mechanism is being utilized, which includes the LISA-RISC (Rapid inter subarray copy) method for transferring data between subarrays. LISA-RISC uses interlinked transistors to transfer data from one subarray to another in the same bank. The method involves issuing a precharge command to precharge the row and activate it in the Row buffer. Then, the RBM (Row buffer movement command) is issued to move the data from one subarray to another, followed by issuing the precharge command to store the data in the required subarray destination row. Using the MASA algorithm's parallel working of subarrays, we can perform parallel transfers at the same time. For instance, data can be transferred simultaneously from subarray 0 to 1 and subarray 2 to 3, and all even to odd-numbered subarray transfers can be performed concurrently. In the next cycle, data can be transferred from subarray 1 to 2 and subarray 3 to 4, and all odd to even numbered subarray transfers can be performed simultaneously. 

% \subsubsection{in-DRAM computing logic}: Our in-DRAM computing logic is based on AMBIT \cite{seshadri2017ambit} \cite{seshadri2015fast} \cite{seshadri2019dram}. AMBIT proposed a technique to perform bulk bitwise operations inside the DRAM array, which can significantly improve performance and efficiency. Building upon AMBIT's approach, SIMDRAM \cite{hajinazarsimdram} provides an architecture that supports complex operations in DRAM by providing compiler and memory controller level support. The SIMDRAM framework consists of three key steps that facilitate the efficient implementation of any desired operation in DRAM while controlling the execution flow of in-DRAM computation transparently from the user.

% The first step in the SIMDRAM framework involves constructing an efficient MAJ/NOT representation of the desired operation from its AND/OR/NOT-based implementation. This step employs logic optimization techniques to minimize the number of logic primitives, thereby reducing computation latency. The SIMDRAM framework derives an optimized MAJ/NOT-based implementation for the desired operation provided by the user.

% The second step is responsible for allocating DRAM rows to the operation's inputs and outputs and generating the necessary sequence of DRAM commands to execute the desired operation. This step converts the MAJ/NOT-based implementation of the operation into AAPs/APs by allocating the designated compute rows in DRAM to the operands and determining the optimized sequence of AAPs/APs that are required to perform the operation. SIMDRAM minimizes the number of AAPs/APs required for a specific operation. The output of this step is a $\mu$Program, which is the optimized sequence of AAPs/APs stored in main memory and used to execute the operation at runtime.

% The third and final step executes the $\mu$Program to perform the operation. When a user program encounters a bbop instruction associated with a SIMDRAM operation, the bbop instruction triggers the execution of the SIMDRAM operation by performing its $\mu$Program in the memory controller. SIMDRAM uses a control unit in the memory controller that transparently issues the sequence of AAPs/APs to DRAM, as dictated by the $\mu$Program. Once the $\mu$Program is complete, the result of the operation is held in DRAM.

% \subsubsection{Optimization}

% In this section, we further exploit the potential benefit from our SSL substrate, proposing extensions enabling meaningful communications among subarrays to optimize the computation process based on a Vector-to-Scalar reduction kernel. The extensions accommodate the inherent mobility of bits supported by LISA\cite{chang2016low} and RowClone\cite{seshadri2013rowclone}, including a Reduction Tree to drive as much computation resource as possible inside a DRAM bank, a Wrap-Around feature to the OBPS bit mapping to increase the throughput for certain algorithms and to control the computation resource usage, and a Dynamic Precision support to obtain better performance for the case when the estimated output precision is higher than the input precision. We further put these optimizations into practice of the real world workload, the Neural Network inference, to demonstrate its feasibility and advantages over applying plain algorithm.

% \subsubsection{Layer Reshape Mechanism for In-DRAM Neural Networks Inference} 

% If we merely operate convolutions of a Neural Network inside DRAM, the results produced by each layer still inevitably need to be move back and forth between the host and the memory, in order to reshape the output feature map into a desired format to be fed into the next layer. \cite{imani2019floatpim} proposes mechanism to support such an inter layer communication for a Non-Volatile Memory based PIM system. Whereas, such a discussion for the Procession-in-DRAM systems have not been brought up comprehensively to our knowledge. Therefore, beyond the convolution, we propose to introduce an efficient mechanism with a minimum hardware modification inside DRAM to perform the in-DRAM layer reshape. Empirically, we found that the layer reshape for the inter layer communication can be decomposed into two steps, matrix row shift, and broadcast. The first step relies on a near bank shifter dedicated to this scenario, and the second step is accomplished through an inter-bank data transfer mechanism proposed by \cite{seshadri2013rowclone}. 
\subsection{Architecture of \prop{}}

% \textit{How and when we use the previous techniques instead of re-explaining them. Check the pLUTo paper.}

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/overview.pdf}
%     \caption{\prop{} overview}
%     \label{fig:overview}
% %    \vspace{-4mm}
% \end{figure}

% \jgl{The first five subsections are not an overview of \prop{}, but background on SALP, LISA, Ambit, and SIMDRAM.}
% \Mayank{Then, I think I should summarize them.}

% \subsubsection{Data Layout}: 
% We have done our analysis of the vertical data layout as proposed in the SIMDRAM framework \cite{hajinazarsimdram}, an end-to-end solution that enables users to implement arbitrary operations in DRAM using the AAP/AP \cite{seshadri2017ambit} command sequences. Our evaluation considers different algorithms implemented in SIMD fashion, with a transposition unit present in the memory controller for converting data into a vertical layout. 

\subsubsection{\prop{} Substrate:}

\prop{} subarray organization is similar to AMBIT \agy{and} DRISA, \agy{resembling} SIMDRAM. There are 1006 D-rows (Data group), 2 C-rows (Control group), \agy{and} 16 B-rows (Bit-wise group which can perform Triple row activation (TRA)) as shown as \circled{1} 
\jgl{Do the circle smaller. And it should have the same appearance as the ones on the figure.} in Fig \ref{fig:high-level}. We implement the SALP (Subarray Level Parallelism) technique \cite{salp} to operate multiple subarrays simultaneously. They employed the MASA (Multitudes of Activated Subarrays) mechanism to enable concurrent activation of multiple subarrays while designating a specific subarray to drive the global bit lines during the next column command. Implementing this technique required DRAM microarchitecture modifications as shown in \circled{2}, including the addition of a designated-bit latch for each subarray, the introduction of a new DRAM command (SA SEL), and the routing of a new global wire (subarray-select). Then, we utilize the Rowclone method \cite{seshadri2013rowclone} - Fast parallel mode (FPM), which copies data within the same subarray by precharging the source row, copying data to the LRB (Local Row Buffer), and then transferring it to the destination row. This mechanism is used to initialize the bulk initialization and transfer data from D-group to B-group rows in our subarray organization. Next, we implemented LISA (Low-cost Interlinked Subarrays) mechanism \cite{chang2016low}, specifically the LISA-RISC method as shown as \circled{3}, to transfer data between subarrays in the same bank. LISA-RISC employs interlinked transistors and a sequence of precharge, RBM, and precharge commands for data transfer. By leveraging SALP-MASA's parallel subarray operations, data can be transferred simultaneously between adjacent subarrays in an alternate manner to activate and transfer data to adjacent \agy{subarrays in parallel} in two cycles. Then we introduce a new Near bank shifter as shown in \circled{4} to employ an efficient data communication scheme across multiple
bitlines to perform \agy{the} bit-shifting operation (More details discussed in Section 4.1.3).  


We implement complex operations in DRAM transparently to the user in our \prop{} compiler:
Step 1) Construct an efficient MAJ/NOT representation of the desired operation, using logic optimization techniques to minimize logic primitives and reduce computation latency as shown in \circled{5}.
Step 2) Allocate DRAM rows to the operation's inputs and outputs, generate DRAM commands, and convert the MAJ/NOT-based implementation into AAPs/APs. This step outputs an optimized $\mu$Program stored in main memory as shown as \circled{6} for runtime execution.
Step 3) Execute the $\mu$Program when encountering the $\mu$-instruction, with a control unit in the memory controller issuing the sequence of AAPs/APs as dictated by the $\mu$Program.  

% To operate multiple bitwise subarrays simultaneously, we will be utilizing the SALP (Subarray level parallelism) technique \cite{salp} proposed earlier. One of the SALP mechanisms we will be using is MASA (Multitudes of activated subarrays). The primary idea behind MASA is to enable the activation of multiple subarrays at the same time while allowing the memory controller to designate one specific subarray to drive the global bit lines during the next column command:

% It overlaps the activation of different subarrays within a bank. Before issuing a column command to any activated subarrays, the memory controller designates one particular subarray whose row buffer should serve the column command. To implement this technique, the following changes need to be made to the DRAM microarchitecture, i) Addition of a designated-bit latch to each subarray, ii) Introduction of a new DRAM command, SA SEL (subarray-select), and iii) Routing of a new global wire (subarray-select).


% \jgl{Do we have an evaluation of total area overhead? Ideally, yes. And it would go at the end of the evaluation section.}

% \subsubsection{Copying and moving data among banks}: We utilize the Rowclone method \cite{seshadri2013rowclone} involving two operations: FPM (Fast Parallel Mode) and PSM (Pipelined Serial Mode). FPM copies data within the same subarray by precharging the source row, copying data to the LRB (Local Row Buffer), and then transferring it to the destination row. PSM extends FPM by transferring data from the LRB to the GRB (Global Row Buffer) and then to a different bank subarray's LRB before copying it to the destination row in another subarray and bank.
% We will be utilizing the Rowclone method proposed earlier \cite{seshadri2013rowclone}, which involves two operations: FPM (Fast parallel mode) and PSM (Pipelined serial mode). FPM is used to copy data from the source row of one subarray to the destination row of the same subarray. This is done by pre-charging the source row and then activating the subarray to copy the data into the LRB (Local row buffer). Then, the destination row is activated, and the data is copied from the LRB to the destination row.

% PSM, on the other hand, is an extension of FPM, where the source row is precharged and activated to copy the data into the LRB. Then, the data is transferred from the LRB to the GRB (Global row buffer) before being copied to a different bank subarray LRB. Finally, the destination row is activated, and the data is copied from the source row of one subarray in one bank to the destination row of another subarray in a different bank.

% \subsubsection{Moving data among subarrays}: The researchers utilized the LISA (Low-cost Interlinked Subarrays) mechanism \cite{chang2016low}, specifically the LISA-RISC method, to transfer data between subarrays in the same bank. LISA-RISC employs interlinked transistors and a sequence of precharge, RBM, and precharge commands for data transfer. By leveraging MASA's parallel subarray operations, data can be transferred simultaneously between adjacent subarrays, such as even to odd-numbered subarrays in one cycle and odd to even-numbered subarrays in the next cycle.
% The LISA (Low-cost interlinked subarrays) \cite{chang2016low} mechanism is being utilized, which includes the LISA-RISC (Rapid inter subarray copy) method for transferring data between subarrays. LISA-RISC uses interlinked transistors to transfer data from one subarray to another in the same bank. The method involves issuing a precharge command to activate the row in the Row buffer. Then, the RBM (Row buffer movement command) is issued to move the data from one subarray to another, followed by issuing the precharge command to store the data in the required subarray destination row. Using the MASA algorithm's parallel working of subarrays, we can perform parallel transfers at the same time. For instance, data can be transferred simultaneously from subarray 0 to 1 and subarray 2 to 3, and all even to odd-numbered subarray transfers can be performed concurrently. In the next cycle, data can be transferred from subarray 1 to 2 and subarray 3 to 4, and all odd to even numbered subarray transfers can be performed simultaneously. 





% \subsubsection{in-DRAM computing logic}: 
% The in-DRAM computing logic is based on AMBIT \cite{seshadri2017ambit} \cite{seshadri2015fast} \cite{seshadri2019dram} and further developed in SIMDRAM \cite{hajinazarsimdram}. The SIMDRAM framework consists of three key steps for implementing complex operations in DRAM transparently to the user:
% 1) Construct an efficient MAJ/NOT representation of the desired operation, using logic optimization techniques to minimize logic primitives and reduce computation latency.
% 2) Allocate DRAM rows to the operation's inputs and outputs, generate DRAM commands, and convert the MAJ/NOT-based implementation into AAPs/APs. This step outputs an optimized $\mu$Program stored in main memory for runtime execution.
% 3) Execute the $\mu$Program when encountering a bbop instruction, with a control unit in the memory controller issuing the sequence of AAPs/APs as dictated by the $\mu$Program. The operation result is stored in DRAM.
% Our in-DRAM computing logic is based on AMBIT \cite{seshadri2017ambit} \cite{seshadri2015fast} \cite{seshadri2019dram}. AMBIT proposed a technique to perform bulk bitwise operations inside the DRAM array, which can significantly improve performance and efficiency. Building upon AMBIT's approach, SIMDRAM \cite{hajinazarsimdram} provides an architecture that supports complex operations in DRAM by providing compiler and memory controller level support. The SIMDRAM framework consists of three key steps that facilitate the efficient implementation of any desired operation in DRAM while controlling the execution flow of in-DRAM computation transparently from the user.

% The first step in the SIMDRAM framework involves constructing an efficient MAJ/NOT representation of the desired operation from its AND/OR/NOT-based implementation. This step employs logic optimization techniques to minimize the number of logic primitives, thereby reducing computation latency. The SIMDRAM framework derives an optimized MAJ/NOT-based implementation for the desired operation provided by the user.

% The second step is responsible for allocating DRAM rows to the operation's inputs and outputs and generating the necessary sequence of DRAM commands to execute the desired operation. This step converts the MAJ/NOT-based implementation of the operation into AAPs/APs by allocating the designated compute rows in DRAM to the operands and determining the optimized sequence of AAPs/APs that are required to perform the operation. SIMDRAM minimizes the number of AAPs/APs required for a specific operation. The output of this step is a $\mu$Program, which is the optimized sequence of AAPs/APs stored in main memory and used to execute the operation at runtime.

% The third and final step executes the $\mu$Program to perform the operation. When a user program encounters a bbop instruction associated with a SIMDRAM operation, the bbop instruction triggers the execution of the SIMDRAM operation by performing its $\mu$Program in the memory controller. SIMDRAM uses a control unit in the memory controller that transparently issues the sequence of AAPs/APs to DRAM, as dictated by the $\mu$Program. Once the $\mu$Program is complete, the result of the operation is held in DRAM.


\subsubsection{Inter-Bank Data Broadcast : }
Originally proposed in \cite{seshadri2013rowclone}, the Pipelined Serial Mode (PSM) performs inter-bank data transfer using the internal bus of the DRAM module. The operation creates a data path through assigning the source (SRC) bank in read mode and the destination (DST) bank in write mode, while disconnecting the internal DRAM bus from the memory channel with the help of augmented Chip I/O logic. Due to the narrow bus bandwidth, only 64 bits of data can be transferred in each cycle between two banks. We found that, with a minimal modification, the PSM can be extended with a technique named Data Broadcast, which communicates the source bank with multiple destination banks. Presented in Figure \ref{fig:PSM}, the destination of the data transfer is changed from one bank to multiple banks (e.g., all other 15 banks). The original logic augmentation to the Chip I/O could maintain the same, since each individual Global Row Buffer (GRB) in each destination bank has enough strength to sense and retrieve information from the data path, without interfering with each other. On the other hand, since the original TRANSFER command \cite{seshadri2013rowclone} contains only one destination bank index, to enable the broadcasting, the command needs to be enhanced to include multiple bank index in a single line. Here, we assume that the column indexes for each destination bank are the same. Derived from \cite{seshadri2013rowclone}, each 64-bits PSM transfer costs 0.8 ns.

Enabled by the modified PSM, the Data Broadcast operation basically generates multiple backups of the transferred data in multiple locations efficiently with low cost. All the backups can be operated concurrently after the transfer. For instance, considering a 2-stage computation where the output of the first stage is the input of the second stage and the second stage exploits parallelism across multiple banks, the Data Broadcast speeds up the original inter-bank data transfer scheme by multiple times according to the parallelism involved in the second stage. In the case of \cite{ferreira2021pluto}, if all the banks contain the same lookup table and perform multiple queries concurrently, the host only needs to load or update the lookup table to one bank and relies on the DRAM module to broadcast the table to all the other banks, saving considerable effort of data communication the host and the memory.

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.43\textwidth]{figures/mPSM.pdf}
    \caption{Modified Pipelined Serial Mode (PSM) \cite{seshadri2013rowclone}}
    \label{fig:PSM}
%    \vspace{-4mm}
\end{figure}

\subsubsection{Bit shifting operation : }

Using the LISA RBM operation, the bit shifting operation within a single bitline can be accomplished straightforwardly within a number of ACTIVATE-PRECHARGE cycles. \cite{li.micro17} adds logic to the DRAM module creating data path across bit-lines, but with a high area overhead. For an in-DRAM arithmetic substrate, an efficient data communication scheme across multiple bitlines is essential for applications with consecutive data manipulation. In this paper, we propose a specialized Near Bank Shifter (NBS) placed adjacent to each DRAM bank, presented in Figure \ref{fig:SHF}. The NBS supports bit-shifting for up to 128-bit data elements deployed with horizontal data layout, and bulk data shifting across up to 128 adjacent bitlines if the vertical data layout is implemented, as in \cite{hajinazarsimdram}. \footnote{Data A moves from bitline A to bitline B, Data B moves from bitline B to bitline C, and so on.}

The NBS supports simple sub-operations like Shift-by-1, Shift-by-2, and Stride-by-2. It contains two sets of latches, controlled by the system clock of the DRAM module. Prior to every operation, all the select signals are set to create a desired path of data flow. During the operation, initially the clock is set high, enabling the Latch A to catch data from the GRB. Once Latch A obtains the original data, the input of Latch B receives the shifted data right away. \footnote{The buffers between Latch A and Latch B are not supposed to contribute a delay longer than half of a clock cycle.} Then, as the clock turns back to low, the Latch B catches the shifted data and feeds it back to the GRB. The area overhead for NBS is estimated at 0.002\% of a bank. The latency preserved for each operation is designed at one clock cycle, 1.25ns. \footnote{The estimation is based on a 128-bit size of the latches, buffers, and MUXs in the NBS. The size can be extended or minimized depending on different practice. }

One real-world application that we evaluated in Section 5 is massively assisted by the NBS, the Neural Networks. The NBS helps to mimic the widely adopted im2col operation \cite{im2col} \cite{trusov2021pim2col} \cite{zhongyu20222im2col} to generate the matrix of GEMM. The process of im2col is described as below. As the filter slides through K rows of the input matrix, where K denotes the kernel size, the converted format for the first group of columns is equivalent to K rows shifted by $K-1$ times and stacked with the original rows on top of each other. Then the filter slides across the next K rows to form the next group of columns, and so on. The NBS reads out the matrix rows to be converted one after another, performs the shifting, and writes them back to the DRAM bank. Since each bank has its own NBS, conversion of multiple matrices can be performed simultaneously, making the in-DRAM im2col operation an even more efficient choice.

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/NBS.pdf}
    \caption{Near Bank Shifter (NBS)}
    \label{fig:SHF}
%    \vspace{-4mm}
\end{figure}


%\jgl{Same as we have in pLUTo and in SIMDRAM, we need an overview section and an implementation section. The explanations in this subsection, for example, are quite detailed. They should go into the implementation section. However, the overview section should give a clear idea of what this component of our substrate is.}


\subsection{Arithmetic approaches}
% As we have explored in the previous section that 1) we can operate on multiple subarrays and banks parallely, 2) we can transfer data between subarrays in same bank as well as different banks. 3) We can horizontally shift the results required and copy it back to the dst subarray and row. 4) we can perform gneral complex operations based on the AP and AAP operations and mechanism provided by SIMDRAM. Based on the above analysis we will derive many bit serial and bit parallel approaches. 

We identified several optimization techniques for \prop{} performance: 1) operating on single and multiple subarrays and banks in parallel, 2) efficient data transfer within and between banks, 3) horizontal shifting of results and copying back to the destination, and 4) using AP and AAP operations efficiently for complex computations. These techniques enable the development of bit-serial and bit-parallel approaches for optimized performance.

We propose two naming conventions for these approaches 1) ABOS (All bits per subarray) for bit-serial methods and 2) OBPS (One bit per subarray) for bit-parallel methods. ABOS involves performing algorithms within one subarray, while OBPS spans bits across multiple subarrays, allowing for parallel computation and intermediate result transfers. This is especially useful for level-based algorithms with O(logn) complexity.


% Based on our previous analysis, we have figured out several ways to optimize the performance of SIMDRAM. Firstly, we can operate on multiple subarrays and banks in parallel, which can significantly increase the speed of our computations. Secondly, we can transfer data between subarrays within the same bank, as well as between different banks, allowing us to efficiently move data around as needed. Thirdly, we can shift the results horizontally and copy them back to the destination subarray and row. This process can save time by eliminating the need to transfer data back and forth between subarrays. Finally, by using the AP and AAP operations provided by SIMDRAM, we can perform complex operations quickly and efficiently.

% Using these techniques, we can develop both bit serial and bit parallel approaches to optimize the performance of our SIMDRAM. By carefully considering the specific requirements of our computations and utilizing the available features of SIMDRAM, we can maximize the speed and efficiency of our data processing.

% We have two naming conventions for the different approaches to optimize SIMDRAM performance. The first one, \textbf{ABOS} (All bits per subarray), refers to bit serial approaches where all the bits are present in one subarray and individual algorithms are performed in one subarray. Multiple subarrays can work in parallel to speed up the computations. The second naming convention is \textbf{OBPS} (One bit per subarray), which refers to bit parallel approaches where one bit is present in one subarray and spanned across multiple subarrays. Bit-parallel algorithms work in which multiple subarrays work in parallel and the intermediate results are transferred from one subarray to another to continue the computation. This approach is based on the fact that algorithms that are performed in O(logn) are generally level-based algorithms in which levels can be computed in parallel.

% We use two naming conventions for the different approaches. 
% \textbf{ABOS} - Bitserial approaches are called as ABOS (All bits per subarray) where all the bits are present in one subarray and individual algorithm is performed in one subarray and multiple subarrays can work parallely. 

% \textbf{OBPS} - Bit parallel approaches are called as OBPS(One bit per subarray) where one bit is present in one subarray and spanned accross multiple subarrays. Here bit-parallel algorithms works in which multiple subarrays work parallely and the intermediate results are transferred from one subarray to another to continue the computation. This can be realized based on the fact that the algorithms which are performed in O(logn) are generally level based algorithms in which levels can be computed parallely. 

% \textbf{Wrap-around OBPS} - This is a mix approach of above two algorithms where multiple bits are stored in one subarray ans spanned accross multiple subarrays. Here bit-parallel approaches are performed in fixed number of subarrays (not all subarrays) and the remaining bits are preformed in the next cycle. This is used to obtain more throughput on cost of latency. 

\subsubsection{Bit serial approaches}
% Bit serial approaches \cite{pudi2014bit} are those approaches where the carry has to be propagated serially and the complexity will be O(n). Based on this we can perform multiplication also serially which will be O($n^2$).

Bit-serial approaches \cite{pudi2014bit} involve carry propagation in a serial manner, resulting in O(n) complexity. This allows for serial multiplication with O($n^2$) complexity.

\textbf{Bit serial adder without multiple subarrays}: This is the same as SIMDRAM addition. Ripple carry adder is used to perform addition where operations are converted MAJ-NOT operations and then in AP and AAP operations. Then optimizations are performed as mentioned in the SIMDRAM and then the final implementation is performed on one single subarray. It takes 8n+1 AP/AAP cycles to compute the addition result where n is the bit precision. This is depicted by figure \ref{fig:bit_parallel_algorithm} (a)

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/code.pdf}
    \caption{Addition algorithm using AP/AAP operations Note: Line 5 is the representation when carry needs to transferred}
    \label{fig:code}
%    \vspace{-4mm}
\end{figure}

\textbf{Bit serial adder with multiple subarrays}: In this approach, we implement the same bit serial addition algorithm used in SIMDRAM but run it in parallel across multiple subarrays to perform vector operations in parallel. We utilized the MASA mechanism of SALP to achieve subarray-level parallelism as shown in figure \ref{fig:bit_parallel_algorithm} (b).

Similarly, bit-serial multiplication can also be performed using this approach by performing addition multiple times. We do not need to perform shift operations during multiplication as the bit serial methodology can take care of it. To do this, we simply precharge and activate a different row to obtain the shift amount and start the iterator from that point.

% In this approach we will implement the same SIMDRAM bit serial addition algorithm which will be running parallelly in multiple subarrays such that vector operations can be performed parallelly. In this, we will use the MASA mechanism of SALP to obtain the subarray level parallelism. We assume that the hardware architecture is present in the DRAM.

% In the same fashion as bit serial addition approaches, bit-serial multiplication can also be performed which is nothing but performing addition multiple times. We dont need to perform shift operations as done in multiplications because that can be taken care by the  bit serial methodology itself because we need just precharge and activate a different row to obtain the shift amount and start the iterator from that point. 

\subsubsection{Bit parallel approaches}
Bit parallel approaches \cite{navarro1998bit} are those approaches where the algorithms are divided into multiple levels and all the operations inside the single level can be done parallelly and then we have to transfer the required results using the LISA mechanism to appropriate subarrays. 

\textbf{Ripple carry bit parallel adder}: In this approach, we implement the same SIMDRAM addition algorithm but work in multiple subarrays parallely for some AP operations, and then it needs to wait for the carry transfer and can perform parallel. As shown in the figure \ref{fig:bit_parallel_algorithm} (c) the independent operations work parallely and wait for the carry transfers from one subarray to another using LISA-RISC isolation transistors. They have to utilize the carry which has to be transferred from the previous subarray (e.g. lets say subarray 0) and then after sending the data the subarray 0 will continue to perform its operations and as soon as subarray 1 is done with the same process with subarray 2. In this case we utilized the full parallelism of subarrays by working parallely and reducing the clock cycles from 8n+1 from the conventional method to 2n + 6. 


% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/Drawing_implementation.pdf}
%     \caption{Different implementation of algorithms. Note: Red boundary denotes computation of one vector. (a) ABOS - One subarray performing one computation. (b) ABOS - Multiple subarrays performing multiple computation. (c) OBPS - All subarrays performing one computation. (d) Wrap around OBPS - Multiple subarrays performing one computation.}
%     \label{fig:bit_parallel_algorithm}
% %    \vspace{-4mm}
% \end{figure}


\textbf{Sklansky bit parallel adder}: In this approach we implement the Sklansky addition which is an O(logn) algorithm that is divided into different levels \mayank{put citation for the figure}. All the operations in one level can be done parallelly as shown in the figure \ref{fig:bit_parallel_algorithm} (c) and then again we have to transfer the intermediate results or carry them to another subarray using the LISA transfers. E.g. We have to transfer the intermediate result from subarray 1 to subarray 2 and 3 and so on. Note : We have not shown the full AP/AAP algorithm as it was very huge.

\mayank{We need to put the table of no of cycles from excel.}

\textbf{Other bit parallel adders}: All the other bit parallel adders like Kogge stone, Ladner Fischer, Brent-Kung, Carry select adders, etc. are designed and evaluated in the same way as we have done the Sklansky adder. We will discuss more on the analysis of these approaches in the microbenchmarks in the evaluation section. 

\textbf{Redundant binary bit parallel adder}: The redundant binary algorithm is a bit-parallel algorithm used for performing the addition of two n-bit numbers. In this algorithm, each bit position in the sum is represented by a pair of redundant bits instead of a single bit. These redundant bits represent the same information as the corresponding single bit, but they also carry additional information which makes it easier to propagate carries through the addition.

To perform the addition using the redundant binary algorithm, we first represent the two n-bit numbers in redundant binary form. We can then perform a bit-parallel addition of the two numbers using a carry-save adder. This gives us the sum in redundant binary form, with two redundant bits for each bit position. Next, we need to propagate the carries through the sum to obtain the final result. This is done by performing a sequence of bit-parallel operations to propagate the carries from one bit position to the next. Specifically, we first compute the carries from the even-indexed positions to the odd-indexed positions, and from the odd-indexed positions to the even-indexed positions as shown in figure \ref{fig:bit_parallel_algorithm} (c) where multiple parallel transfers can take place. We then repeat this process, propagating the carries from each even-indexed position to the next odd-indexed position, and from each odd-indexed position to the next even-indexed position. To achieve this we have utilized the parallel activation of subarrays from MASA mechnaism and LISA transfers which performs the transfers in ACT-PRE-RBM command sequences. Using this carries have been propagated parallely using LISA shifts, we obtain the final result in redundant binary form. 

The redundant binary algorithm has a constant time algorithm complexity of O(1), which makes it very efficient for large inputs. However, it requires more bits to represent the sum than the original n-bit inputs.

% It is also a bit parallel algorithm of the complexity of O(1) but the size of the input is increased to 2 times the bit precision as compared to 2's complement.  
% \mayank{Explain redundant binary algorithm}
% As shown in the figure, all the operations are being performed parallelly and then the carry 1 is transferred parallelly from the even indexed subarray to the odd indexed subarray and odd next odd indexed subarray to even indexed subarray parallelly as discussed in the modified LISA mechanism overview. Then we again perform the computation parallelly and then send carry 2 to the next subarrays parallelly just like before. In this way, we can perform computation parallelly. The no of AP/AAP operations is quite large as compared to the 1-bit addition operation as shown in Figure but it needs to be done only once, owing to its constant time algorithm complexity. In this case, the number of AP/AAP clock cycles turns out to be x.   

\textbf{Shift and add bit parallel multiplier}: The conventional shift and add multiplication algorithm involves having the operands initially present in their respective subarrays. The partial product is then generated and transferred to the correct subarray to obtain the required shift amount. Once the partial products have been shifted, any bit parallel adder can be used to perform the addition operation.

For example, consider a 4-bit multiplication,  initially, the operands are present in subarrays 0-3. The partial product is then generated and shifted in parallel using LISA shifts to their respective destination subarrays. At this point, each subarray has their partial products, which then need to be added. This can be done by performing 8-bit precision bit parallel addition four times to obtain the final multiplication results.

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/multiplication.pdf}
%     \caption{Shift and add bit parallel partial product generation
%     Note: Steps written in the figure doesn't correspond to cycles.}
%     \label{fig:multiplication}
% %    \vspace{-4mm}
% \end{figure}

\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/Drawing_implementation.pdf}
    \caption{Different implementation of algorithms. Note: Red boundary denotes computation of one vector. (a) ABOS - One subarray performing one computation. (b) ABOS - Multiple subarrays performing multiple computation. (c) OBPS - All subarrays performing one computation. (d) Wrap around OBPS - Multiple subarrays performing one computation.}
    \label{fig:bit_parallel_algorithm}
%    \vspace{-4mm}
\end{figure}


% It is the conventional shift and add multiplication algorithm in which operands are intially present in their subarrays as shown in the figure and then the partial product is generated and transferred to the correct subarray to obtain the shift amount required and then it can be followed by any bit parallel adder. E.g. as shown in figure we have considered a 4 bit multiplication in which initally operands are present in subarray 0-3. Then the partial product is generated and shifted parallely using LISA shifts to their destination subarrays. Now each subarray has their partial products which needs to be added and hence we will perform 8-bit precision addition 4 times to get the multiplication results. 

\textbf{Karatsuba bit parallel multiplier}: The modified version of the shift and add multiplication algorithm involves dividing the operands into lower and upper halves and then using a bit parallel multiplier to generate the partial results for each segment. These partial results are then combined using LISA shifts to use them in the Karatsuba algorithm. Assuming X and Y are two n-bit operands, Xl and Yl represent the lower bits of X and Y, while Xr and Yr represent the higher bits of X and Y. According to the Karatsuba equation, XY = $2^n$XlYl + $2^\frac{n}{2}$[(Xl+Xr)(Yl+Yr) - XlYl -XrYr] + XrYr.

To implement this algorithm in SIMDRAM, all the multiplications can be divided and performed using the Karatsuba algorithm, and the additions can be performed using any bit-parallel algorithm. The required shifting can be done using LISA shifts, as explained in the previous results.

% It is the modified version of shift and add multipliation algorithm in which we will divide the operands into lower half and upper half and then perform shift and add bit parallel multiplier to individual segments to generate the partial results and again will combine them by LISA shifts to use it in the karatsuba algorithm. Assume X and Y are two n-bit operands and Xl, Yl are lower bits of X and Y and Xr, Yr are higher bits of X and Y, therefore according to karatsuba equation is given by XY = $2^n$Xl*Yl + $2^\frac{n}{2}$*[(Xl+Xr)*(Yl+Yr) - Xl*Yl -Xr*Yr] + Xr*Yr. Now in this equation all the multiplication can again be divided to be performed by karatsuba algorithm and addition can be performed by any bit parallel algorithm. Shifting can be taken care LISA shifts as explain in previous results. In this we can perform Karatsuba multiplication also. 

\subsection{Optimization}

\subsubsection{Wrap Around OBPS} 

The drastically limited throughput acts as the major performance bottleneck for the bit-serial algorithm with OBPS. For 64-bit numbers, one SIMD lane can only support one addition at a time. Assuming we store the 64-bit numbers with two-bits-per-subarray, instead of the regular OBPS, then the computation resource is reduced by half, while the throughput per lane is doubled. For the carry propagation, as Figure \ref{fig:RED_WA} suggests, the carry bit generated from the \nth{4} bit position is propagated to the first subarray, where the \nth{5} bits are located. Such a bit propagation contributes to the only overhead for this multi-bits-per-subarray bit mapping, or namely Wrap-Around OBPS. 

The bit-parallel algorithm is also compatible with the Wrap-Around OBPS. However, such an extension limits only a segment of data (e.g., 4 bits of an 8-bit number) to be accessed per operation, meaning each parallel computation is divided into a few consecutive steps, degrading the performance consequently. 

Besides, the Wrap-Around extension can also benefit the scenario when the computation resource within the DRAM bank is limited. Considering an occasion when there is only 4 available subarrays but for 64-bit computation, the Wrap-Around extension will work as a major enabler in this case. 

\subsubsection{Dynamic Precision} 

A common approach to tolerate overflow of reduction for low precision numbers is to use a higher precision accumulator \cite{QAT}. In this way, the accuracy of the computation is always guaranteed, while sacrificing certain amount of performance per computation. Using the inherent capability of our In-DRAM arithmetic substrate, we propose a Dynamic Precision feature to our reduction kernel to reasonably mitigate this kind of performance overhead with computation accuracy assured.

Generally, the in-DRAM Dynamic Precision arithmetic works as follows. Assuming a vector containing N X-bit numbers, it is firstly grouped into N/2 pairs and performed with a series of (X+1)-bit additions, reserving an extra bit position for the potential last carry bit. Then, the N/2 (X+1)-bit intermediate results are further grouped into N/4 pairs and performed with (X+2)-bit additions. The process iterates until the final reduction result is produced. Hence, the output precision will depend on the vector size, instead of being determined with a high precision in advance. 

For the SIMDRAM arithmetic, the extra bit position reserved can be seen as another DRAM row inside the subarray where the addition is taken place. For the bit-serial arithmetic with Wrap-Around OBPS, the reservation is wrapped into the subarrays assigned initially to the operands. For the bit-parallel arithmetic, the reservation requires to a new subarray. Whereas, conversely, the throughput of the bit-parallel arithmetic will be further constrained yet.  
Furthermore, for the reduction kernel, the Dynamic Precision is designed with two modes, automatic mode and user-define mode. In automatic mode, the output precision depends on the vector size, calculated as $ceil(log2(Vector Size))$. In user-define mode, the user should give a desired output precision to the API, and we assume that the user has the control of the input excluding the possibility of overflow. 

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.12\textwidth}
%          \centering
%          \includegraphics[width=0.92\textwidth]{figures/red_wa_demo.pdf}
%          \caption{}
%          \label{fig:RED_WA}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.12\textwidth}
%          \centering
%          \includegraphics[width=0.7\textwidth]{figures/red_dyn_demo.pdf}
%          \caption{}
%          \label{fig:RED_DYN}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.12\textwidth}
%          \centering
%          \includegraphics[width=1\textwidth]{figures/red_wa_dyn_demo.pdf}
%          \caption{}
%          \label{fig:RED_DYN_WA}
%      \end{subfigure}
%         \caption{OBPS Bit Mapping Extension for (a) Wrap-Around, (b) Dynamic Precision, (c) Wrap-Around and Dynamic Precision}
%         \label{fig:three graphs}
% \end{figure}



